Differentiable Combinatorial Scheduling at Scale

This paper addresses the complex issue of resource-constrained scheduling, an NP-hard problem that spans critical areas including chip design and high-performance computing. Traditional scheduling methods often stumble over scalability and applicability challenges. We propose a novel approach using a differentiable combinatorial scheduling framework, utilizing Gumbel-Softmax differentiable sampling technique. This new technical allows for a fully differentiable formulation of linear programming (LP) based scheduling, extending its application to a broader range of LP formulations. To encode inequality constraints for scheduling tasks, we introduce \textit{constrained Gumbel Trick}, which adeptly encodes arbitrary inequality constraints. Consequently, our method facilitates an efficient and scalable scheduling via gradient descent without the need for training data. Comparative evaluations on both synthetic and real-world benchmarks highlight our capability to significantly improve the optimization efficiency of scheduling, surpassing state-of-the-art solutions offered by commercial and open-source solvers such as CPLEX, Gurobi, and CP-SAT in the majority of the designs.

==> icml2024/3-approach.tex <==
\section{Approach}
\label{sec:approach}

%In this work, we intend to solve the scheduling problem for SDC based on a directed-acyclic graph (DAG) setup for simplification. Specifically, the optimization objectives of scheduling can be defined as follows: \textbf{Given}: (1) A DAG $G(V,E)$ where $V$ represents the set of nodes, and $E$ represents the set of edges; (2) A set of scheduling constraints, which may include dependency constraints, memory constraints, etc. \textbf{Objective}: Construct an optimal schedule $S = s_0,s_1,...s_i$, $i \leq |V|$, where $s_i$ represents the scheduled stage of node $v_i$. 

%In this work, our primary objective is to seamlessly integrate SDC-based and Linear Programming (LP) models based scheduling \cite{brglez1989combinational,leiserson1991retiming} with conditional sampling-based differentiable discrete optimization for task scheduling. 

We propose a novel \fixme{differentiation} \zz{let's use the term differentiable approach; it's not like we are actually differentiating SDC} approach that \textit{compactly encodes} our targeted scheduling problem defined in Section \ref{subsec:schedule}, which can also be applied to a variety of important scheduling problems on dataflow graphs. Specifically, our primary objective is to seamlessly integrate (a) SDC scheduling formulation, which handles the dependencies, and (b) LP models that handles the targeted minimization objectives, with conditional sampling-based differentiable discrete optimization. As a result, our proposed approach will be able to derive the fully differentiable formulation of scheduling problems that can be formulated in SDC with LP based cost models. Note that this approach is specifically designed to address the discrete complexities inherent in these graph structures. To navigate through this intricate solution space, we introduce a novel \textit{conditional Gumbel-Softmax} (GS) reparameterization technique. The remainder of this section will outline the formulation of the targeted scheduling problem in a combination of SDC and LP programming forms, detailing the (1) definition of the search space, (2) modeling of dependencies, and (3) cost metrics (optimization objectives). Following this, we will present our differentiable approach, aligning it with these three key components.

%The node set $V$ will be allocated to $S$ that satisfies all scheduling constraints. Among the existing scheduling problems, we take into account two optimization objectives: memory and communication cost minimization. In this section, we will carry out two methods dedicated to solving this problem: Integer Linear Programming (ILP) and our proposed differentiable scheduling framework utilizing Gumbel Softmax.

\subsection{SDC Formulation and Cost Objectives of the Targeted Scheduling Problem}\label{sec:ilp}
% As shown in Figure \ref{fig:case_study}a, $N$ various tasks are formulated as $N$ distinct nodes connected by directed edges which represent the task dependencies. 
We intend to schedule the node set $V$ on $L$ scheduling locations (or schedule stages) to achieve the minimum resource (memory) among the stages and minimum communication cost resulting from inter-stage communications. Note that, we allow chaining which indicates the scheduled stage of the child node cannot be earlier than the parent node (on the same stage is allowed).

\paragraph{(1) Search space and dependency constraints} The first step in scheduling model is to define the search space, which involves enumerating all feasible schedules. For each node in $G$, each potential schedule is represented as a point in an $L$-dimensional space, where $L$ corresponds to the upper bound of latency constrain (Eq. \ref{eq:space})
\begin{equation}  
      \begin{aligned}       \sum_{j=0}^{L-1} s_{ij} &= 1 \quad \forall i \in \{0, 1, \ldots, |V|-1\},
    \end{aligned}
    \label{eq:space}
\end{equation}
\noindent where $s_{ij}$ is a binary variable indicating the scheduling choice of node $v_i$ on the stage $j$. 

With this formulation, the schedule of each node can be determined by summing up the choice on any stage with the relative stage number, which is:
\begin{equation}  
    \begin{aligned}
        \sum_{j=0}^{L-1} j \cdot s_{ij} &= s_i \quad \forall i \in \{0, 1, \ldots, |V|-1\}.
    \end{aligned}
\end{equation}
\noindent where integer variable $s_i$ is the schedule of node $v_i$.

A critical aspect of scheduling is respecting the dependencies among the operators in $G$. Specifically, these dependencies are translated into linear inequalities, which ensure that the resulting schedule adheres to the necessary precedence and resource constraints, maintaining the integrity of the dataflow. Specifically, the inequality constraints can be summarized w.r.t the edges $E$, 
\begin{equation}  
    e: s_k - s_t \leq 0 \quad \forall e \in E.
\end{equation}
\noindent where each edge \( e \) connects node \( v_k \) to node \( v_t \), and \( E \) is the set of edges. The term \( s_k \) and \( s_t \) represent the scheduled stages for nodes \( v_k \) and \( v_t \), respectively.


\paragraph{(2) Modeling of the two cost metrics}  As discussed in Section \ref{subsec:schedule}, we target the scheduling problem of minimizing the peak memory usage as well as the cross-stage communication cost, where the cost metrics can be assessed uniquely w.r.t a given schedule. For instance in Figure~\ref{fig:sdc-example}, consider a schedule where $v_0$, $v_1$, and $v_2$ execute in the first cycle, while $v_5$ executes in the last cycle. The communication cost is then calculated as the sum of all data transferred between stages $I_0$ and $I_1$. As for the memory cost, the peak memory refers to the maximum memory used across all cycles. 

The LP modeling typically necessitates additional inequalities to accurately represent various cost components, such as communication costs and peak memory usage. To define the upper bound of the per-stage memory cost (peak memory), we introduce extra inequality constraints. These constraints calculate the memory bound for each stage and identify the maximum among all stages. A new variable, $r_{l}$, is introduced to denote the current memory bound of stage $l$. The relevant equations are as follows:
\begin{equation}  
\small
    \begin{aligned}
        \sum_{i=0}^{|V|-1} rv_{i} \cdot s_{ij} &= r_{j} \quad \forall j \in \{0, 1, \ldots, L-1\}, \\
        \bigwedge (r_j - r) &\leq 0 \quad \forall j \in \{0, 1, \ldots, L-1\}.
    \end{aligned}
    \label{eq:peak_mem}
\end{equation}
Here, $rv_{i}$ represents the required memory of node $v_i$ and $r$ is the memory upper bound found by the scheduling. 

For communication costs, the model needs to account for costs incurred in each inter-stage transition, denoted as $m_0, m_1, \cdots, m_{L-2}$. Inter-stage communication costs are introduced when two connected nodes are scheduled in different stages. These costs are aggregated into the corresponding communication cost variable $m_i$. The formulation is as follows:
\begin{equation}  
    \begin{split}
        \sum_{b=0}^{|E|-1} \Bigg( c_{b} \cdot \Bigg(\sum_{a=0}^{i} s_{ka}\Bigg) \cdot 
        \Bigg( \sum_{h = i+1}^{L-1} s_{th}\Bigg) \Bigg) = m_{i} \\ \quad \forall i \in \{0, 1, \ldots, L-2\}.
    \end{split}
    \label{eq:communication}
\end{equation}
In this equation, each edge $e_b$, for $b \in \left[ 0, |E|-1 \right]$, connects node $v_k$ to node $v_t$, with $c_{b}$ as the communication cost of the edge $e_b$ and $|E|$ representing the total number of edges.




%\subsection{ILP formulation}
\paragraph{(3) Optimization objectives}
Finally, the optimization objectives will be given to complete the scheduling problem. %The state-of-the-art ILP-based method has achieved outstanding performance in obtaining an optimized schedule of multiple tasks. 
For example, targeting peak memory and communication cost aware scheduling, we will leverage Equations \ref{eq:peak_mem}--\ref{eq:communication} to form a complete cost objective:
\begin{equation}  
    \text{min} \sum_{i=0}^{L-2} m_i + \mathcal{R} r 
\end{equation}
\noindent where $L$ is the total stage number, and $\mathcal{R}$ is a ratio parameter to differentiate between the memory upper bound  $r$ and the sum of $m_i$ to impact on the optimization emphasis. In this work, we apply a relatively large ratio $\mathcal{R}$, focusing more on memory minimization than communication cost minimization.

%The scheduling can take lots of expert efforts, heavy computation, and runtime overhead due to (1) the discretion of scheduling selections; (2) the complex dependency between scheduled stages, impeding the fixable, efficient and comprehensive explorations and design automation on modern computing platforms such as GPU.

\subsection{Differentiable Scheduling Formulations}
% \zz{Section title seems misleading. The previous sections only talk about SDC and LP, instead of ILP. I suggest we use ``Differentiable Scheduling Formulations''}

In this section, we present the core of our research: a novel approach to differentiable modeling for combined SDC scheduling formulation. Echoing the structure used in Section \ref{sec:ilp}, we will introduce our formulations into three fundamental components: (1) defining the search space within a vector space, (2) differentiating inequalities, and (3) formulating differentiable cost (loss) functions. This breakdown will help clarify how our approach uniquely addresses the challenges in scheduling optimization. Note that our proposed formulation specifically targets discrete differentiation for the integer inequality constraints, since all schedule variables and cost variables are integers.
%Beyond the illustrated dependence, communication optimization, and cycle time constraints, ILP scheduling formulation has the capability to encode various other latency and relative timing constraints. The overall constrained scheduling problem can be constructed by incorporating a linear objective function that models either the performance or cost of the design. However, the use of a linear objective form places practical limitations on scheduling optimization, as it can only provide an approximation of the cost through a weighted sum. To overcome these deficiencies, we propose to develop novel differentiable solving approach that uniquely encodes the ILP scheduling constraints in fully differentiable formats, using Gumbel-Softmax based sampling method.

%\paragraph{(1) Search space vectorization}  -- Given a vector \(\overrightarrow{x}\) in \(\mathbb{R}^n\), we call \(\overrightarrow{x}\) a one-hot vector if %satisfies the indicator function:
%{\small
%\[
%{1}_A(x_j) :=
%\begin{cases}
%1 &\text{if } j = i, \\
%0 &\text{if } j \neq i.
%\end{cases}
%\]
%}
%\paragraph{(1) Search space vectorization}  -- Given a vector \(\overrightarrow{x}\) in \(\mathbb{R}^n\), we call \(\overrightarrow{x}\) as the probability base of scheduling decision for a given node. Let \(\overrightarrow{s}\) be the sampled decision generated via GS in one-hot encoding, i.e., \(\overrightarrow{s}\) has only one 1 in the \(i^{th}\) coordinate and 0's elsewhere, \(\overrightarrow{s}\)=GS(\(\overrightarrow{x}\)). The integer value corresponding to a given discrete samples of \(\overrightarrow{x}\) via GS is denoted as \(i\), where \(i\) is returned with \texttt{argmax}(\(\overrightarrow{s}\)). 
%As a result, for any schedule variable vectorized with \(\overrightarrow{x}\) in \(\mathbb{R}^n\), its corresponding integer solution space is defined as \(i\), where \(i \in [0, n-1]\) and $n$ is latency upper bound. 


%Additionally, let \(\overrightarrow{s}\) represent a vectorized version of the variable \(s\) from an SDC, such that each \(s_i\) in \(\overrightarrow{s}\) represents an integer in the search space for \(s\). 
%Note that the search space may not always be in the positive integer range. %(e.g., retiming SDC). 
%Beside, we can see that the complexity of the vectorization of each variable is linear to the upper bound search space, which could cause high memory usage. Thus, the vectorization range cannot be limited and fixed to the vectorization size. Therefore, we propose to implement a pivot-based vectorization factor -- 

\paragraph{(1) Search Space Vectorization} Consider a vector \(p\) in \(\mathbb{R}^n\), representing the probability basis of scheduling decisions for a given node. The sampled decision, denoted as \(\overrightarrow{s}\), is generated via Gumbel-Softmax (GS) in one-hot encoding. This means \(\overrightarrow{s}\) contains a single '1' in its \(i^{th}\) coordinate and zeros elsewhere, defined as \(\overrightarrow{s}\) = GS(\(p\)). The integer value corresponding to the discrete sample of \(p\) via GS is denoted as \(i\), obtained using \texttt{argmax}(\(\overrightarrow{s}\)). Therefore, for any scheduled variable vectorized as \(p\) in \(\mathbb{R}^n\), its corresponding integer solution space is defined as \(i\), where \(i \in [0, n-1]\) and \(n\) is the latency upper bound.

In the context of an SDC-encoded schedule, the solution values for each variable are defined within its vector representation, i.e., \(s_i \in \mathbb{R}^n\), with \(s_i \in [0, n-1]\). For each variable \(s_i\), the value range is from \(0\) to \(n-1\). In our implementation for a DAG \(G(V, E)\)—where \(V\) is the set of nodes and \(E\) the set of edges—and given the expected scheduling upper bound \(L\), each schedule variable resides in \(\mathbb{R}^L\). Consequently, the total trainable parameters are in \(\mathbb{R}^{|V| \times L}\). This vectorization establishes a bijection between each integer value and its corresponding one-hot vector. Considering all variables in the SDC, the search space can be effectively represented by the tensor product of these one-hot vectors.

 

\paragraph{(2) Differentiation of Inequality Constraints} In the combinatorial optimization of scheduling \(|V|\) nodes, the selection of schedules is constrained by \(|E|\) dependency vectors. Our differentiable models must recognize and adhere to these dependency constraints, typically defined as inequalities. To encode these inequalities in a differentiable manner, we utilize the \texttt{cumsum} function. For an SDC variable represented as a one-hot vector \( s_i \), the transformation using \texttt{cumsum} yields \( \texttt{cumsum}(s_i) \), converting \( s_i \) into its cumulative sum representation. Generally, the cumulative sum of a vector \( v = [v_0, v_1, ..., v_n] \) is \( v' = [v_0, v_0 + v_1, ..., \sum_{i=0}^{n} v_i] \). For one-hot vectors, this transformation indicates the feasible space for subsequent operations.

Given a difference constraint \(s_i - s_j \leq c_{ij}\), we express it in vector form as \( \overrightarrow{s_i} \xrightarrow{c_{ij}} \overrightarrow{s_j} \), where \(\overrightarrow{s_i}\) is the sampled discrete solution of \(s_i\). We define a transformation \(T_{\leq}: \mathbb{R}^n \times \mathbb{R} \to \mathbb{R}^n\) for the "\(\leq\)" constraint:  
\begin{equation}  
\mathbf{T_{\leq}}(\overrightarrow{s_i}, c_{ij}) = \texttt{cumsum}(\overrightarrow{s_i} + \overrightarrow{c_{ij}})
\end{equation}
This transformation \(T_{\leq}(\overrightarrow{s_i}, c_{ij})\) effectively constrains the solution space for \(s_j\), represented as \(\overrightarrow{s_j}\). For example, for the constraint $s_0 - s_1 \leq 0$, with $s_0, s_1 \in \mathbb{R}^3$ and the initial sampling of $s_0$ as [0,1,0] ($s_1=1$), $T_{\leq}$ will be [0,1,1]. This implies that if $s_1=0$, $s_0$ can only be sampled as 1 or 2 due to the inequality constraint. The solution for \(s_j\) should thus be sampled within the space indicated by \(T_{\leq}\).


\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{icml2024/figs/framework.pdf}
    \caption{The implementation overview of our differentiable scheduling. $p$ indicates the probability vector for each node during GS-enabled differentiable  optimization; $T$ indicates the dependency constraints from the parent nodes; $S$ indicates the scheduled stage for the node. (a) The search space vectorization and GS initialization. (b) The legal scheduling after applying the dependency constraints. (c) The scheduling is optimized with GS-enabled differentiable optimization.
    }
    \label{fig:framework_overview}
\end{figure*}


We introduce the \textit{Constrained Gumbel Trick}, extending our model capability to handle integer linear and inequality constraints. We use \(T_{\leq}\) in conjunction with Gumbel distribution sampling:
\begin{equation}  
y'_i=\frac{\exp((\log(p_i)+g_i)/\tau)}{\sum_j \exp((\log(p_j)+g_j)/\tau)} \cdot \mathbf{T_{\leq}}, \quad g \sim \text{Gumbel}(0,1)
\end{equation}
This ensures that the sampling always satisfies the constraints.

\begin{lemma}[Transformation Ensures SDC Inequality]
For the inequalities \( s_i - s_j \leq c_{ij} \), the transformation \( T_{\leq} \) ensures any sampled vector space for \( s_j \) satisfies the inequality.
\end{lemma}

\begin{proof}
Consider any arbitrary constraint \( s_i - s_j \leq c_{ij} \). The transformation \( T_{\leq} \) applied to \(\overrightarrow{s_i}\) restricts the feasible vector space for \(\overrightarrow{s_j}\). Any vector \( \overrightarrow{s_j} \) sampled from this space will satisfy the inequality when converted back to integer values via the bijection.
\end{proof}


\paragraph{(3) Loss function and optimization} The optimization process in our model focuses on finding the optimal scheduling solutions within the defined constraints. The core of this process is the Constrained Gumbel Trick, which we apply to the vectorized representations of scheduling decisions. Firstly, we calculate the logits for each scheduling decision, then we incorporate these logits into the Gumbel Softmax (GS) function with our constraint transformations to obtain the sampling probabilities. The process can be mathematically represented as follows:

Let \(\overrightarrow{s}\) be the vector representation of a scheduling decision for a node. We apply the Gumbel Softmax function with the Constrained Gumbel Trick to get the sampling probability:
\begin{equation}  
P_k = \text{GS}(\mathbf{T_{\leq}}(\overrightarrow{s}, {c}); \tau),
\end{equation}
where \( P_k \in \mathbb{R}^L \) and \( P_k^i \in [0, 1] \) for each \( i \in [0, L-1] \) with \( L \) being the scheduling depth upper bound. Here, \( \mathbf{T_{\leq}} \) represents the transformation for inequality constraints and \( \text{GS}(\cdot; \tau) \) is the GS function with temperature \( \tau \).

The probability of selecting a scheduling solution can be calculated by considering both the conditional probabilities under the constraints and the overall probability of the solution being feasible. For a scheduling solution \( k \), the probability \( P(i) \) for a node \( i \) can be computed as:
\begin{align}
P(i) &= P(i|k) \cdot P(k) \\
     &= P(i|k) \cdot p(cl(i)),
\end{align}
where \( P(i|k) \) is the conditional probability of choosing node \( i \) given the scheduling solution \( k \), and \( p(cl(i)) \) represents the probability of the scheduling class \( cl(i) \) being feasible under the given constraints.


 %Given the use of GS reparameterization, \(\mathcal{L}\) can be treated as a differentiable function of the embedding table \(E\) and the mapping function parameters \(\theta\). Consequently, we can employ gradient descent to minimize \(\mathcal{L}\) with respect to \(E\) and \(\theta\). Specifically, our targeted scheduling problem is formed by two loss components: memory loss and communication loss.


Finally, we integrate a differentiable cost function \(\mathcal{L}(\theta)\) that takes \(\theta\) and \(P(i)\) as inputs. To minimize memory usage in latency-fixed scheduling, we define the memory loss function \(\mathcal{L}_{e}\), which includes the entropy of scheduled nodes over \(L\) stages:
\begin{equation} 
    \mathcal{L}_{e} = -\sum_{i=0}^{L-1} \frac{N_{i}}{M}\log \frac{N_{i}}{M}
    \label{equ:loss_entropy}
\end{equation}
where \(N_{i}\) represents the memory of all nodes at the \(i\)-th stage, and \(M\) is the total memory of all nodes. Assuming uniform memory requirements for each node, \(N_{i}\) is equivalent to the number of nodes at the \(i\)-th stage, and \(M = |V|\), the total node count. Minimizing \(\mathcal{L}_{e}\) aims to evenly distribute the required memory across stages. The effectiveness of this entropy-based approach for scheduling memory usage optimization is proven in~\cite{wang2010multi}.



Furthermore, to take account the minimization of communication cost, we add $\mathcal{L}_{c}$ into the loss functions. In this context, we simply formulate the communication cost as the mean of total cost over all the inter-stages, i.e.,
\begin{equation}
    \mathcal{L}_{c} = \frac{1}{\sum_{b=0}^{|E|-1}c_{b}} \sum_{i=0}^{L-2} m_i
\end{equation}
\noindent where $m_i$ is the accumlated communication cost for all edges on each inter-stage $i$, $c_{b}$ is the communication cost introduced by edge $e_b$. The final loss is then defined as
\begin{equation}  
    \mathcal{L} = \lambda \mathcal{L}_{e}+\mathcal{L}_{c}
\end{equation}
\noindent where $\lambda$ is a factor similar to the ratio in LP formulation.
%Different from the ILP formulation, we need to formulate the communication cost while maintain the differentiability. As mentioned before, the schedule of each node is represented as a one-hot vector. For edge $e_b$ connecting node $v_k$ and node $v_t$, we have the following formulation,
\iffalse
\begin{equation}  
    m_i = \sum_{b=0}^{|E|-1} m_{ib}
\end{equation}
\begin{equation}  
\begin{split}
    m_{ib} = &\texttt{sum}(\overrightarrow{s_k} \times (\overrightarrow{1}-\texttt{cumsum}(\mathcal{T}_i))) \cdot \\
    &\texttt{sum}(\overrightarrow{s_t} \times \texttt{cumsum}(\mathcal{T}_i)) \cdot c_{b}, \\
    &\forall b \in \{0, 1, \ldots, |E|-1\}
\end{split}
\end{equation}
\noindent where $m_{ib}$ is the communication cost introduced by edge $e_b$ crossing inter-stage $i$, and $\mathcal{T}$ is a modified indentity matrix of size $L \times L$ by removing the first row.$\overrightarrow{s_k}$ is the schedule vector of node $v_k$ and $\overrightarrow{s_t}$ is the schedule vector of node $v_t$. $\texttt{sum}$ is the summation of all elements in the result vector. In this case, we can model the communication cost loss in a differentiable way. 
\fi

\iffalse 
Moreover, similar to the ratio setup in ILP formulation, to balance the gradients from entropy and communication loss, we introduce a regularization factor $\lambda$, i.e.,
\begin{equation}  
    \mathcal{L} = \lambda \mathcal{L}_{e} + \mathcal{L}_{c}
    \label{equ:loss}
\end{equation}
We will adjust the regularization factor $\lambda$ based on graphs of different sizes with given pre-defined stages $L$ for efficient and better optimization performance.
\fi 

%Note that , where $\mathcal{L}$ can be any differentiable cost function other than .....

%In this work, we propose an end-to-end differentiable scheduling framework ScheduleNet with dependency modeling for full design automation on GPUs based on Gumbel-Softmax. 

\paragraph{Implementation} The overview of the differentiable optimization for SDC is shown in Figure \ref{fig:framework_overview}. First, each variable (node) is initialized with the vectorized search space, i.e., given 3 available stages and thus 3-dimensional vector, while made differentiable with Gumbel-Softmax (GS) (Figure \ref{fig:framework_overview}(a)). Note that, the root nodes ($v_{0}$, $v_{1}$ and $v_{2}$) are initialized with the distribution biased to the first stages in GS to provide enough search space for optimization, while other nodes are initialized randomly. Then, the constraints $T$ are applied to the initialized $p$ to produce the legal one-hot scheduling $S$. For example, for $v_{5}$, even though the first stage shows the highest probability in $p_{5\_0}$, its feasible search space is constrained by its parents $v_{4}$ and $v_{3}$ with $T_{5\_0}=[0, 1, 1]$ and the legal scheduling is then selected within the feasible space with the highest probability, i.e., the second stage. In each optimization iteration, in the forward path, the loss function is computed by the legal one-hot scheduling $S$ to guarantee its legalization and the scheduling is optimized with the backward propagation through the probability vector $p$ provided by GS to make it differentiable. By updating the probability vector $p$, the one-hot scheduling will be updated accordingly in the next iteration to realize the differentiable iterative optimization. We illustrate the training process of our approach as shown in Algorithm \ref{alg:training} for a given graph $G(V,E)$ with a targeted latency $L$, in the APPENDIX \ref{sec:appendix_impl}.





 


==> icml2024/3-b-approach-example.tex <==

\subsection{Examples}
Specifically, this work mainly involves three steps: (1) formulating the scheduling over $L$ stages as one-hot representation of $L$ dimensions; (2) modeling the dependencies between stages for the dependency awareness during backpropagations; (3) composing the reasonable loss functions. The full differentiable with the awareness of stage dependencies scheduling modeling in our framework enables the gradient-based optimizations with efficient scheduling exploration with versatile optimization targets. In this section, we will demonstrate the formulations in the framework with the illustration by a case study as shown in Figure~\ref{fig:case_study}, where our target is to schedule the network with 5 nodes on $L=3$ stages with minimum memory and communication cost required. 


\begin{figure}[!htb]
    \centering
    \includegraphics[width=1\linewidth]{icml2024/figs/case_study-crop.pdf}
    \caption{The case study for 5 nodes scheduled on 3 stages. (a) The given graph numbered following topological order. (b) The initialization over 3 stages of nodes. For each node, the scheduling is initialized as a 3-dimensional vector. The root nodes are initialized at the first stage, other nodes are random initialized. (c) The dependency $D$ from parent nodes and scheduling decision in the forward pass. }
    \label{fig:case_study}
\end{figure}


\subsubsection{Differentiable Discrete Selection}

First, the schedule stage for each node is formulated as an one-hot representation, i.e., for each node, its scheduling is a vector of dimension $L$, where $L$ is the number of total available stages. For the initialization, we set the root nodes, i.e., the nodes without parent nodes, at the first stage. Note that the initialization for roots is also trained for the optimization target during the training process. 
The scheduling stages for other nodes are initialized with a random $L-$dimensional vector, as the stages of other nodes are dependent on the stages of its parent nodes and the corresponding dependencies in the structure.  
For example, in Figure~\ref{fig:case_study}, when $L=3$, the root nodes $1, 2$ are initialized as $[1, 0, 0]$ and other nodes are random initialized for a 3-dimensional vector.

Then, the one-hot represented scheduling is formulated as differentiable selections by Gumbel-Softmax with the parameters $g_{i}$ and $\pi_{i}$ in Equation~\ref{equ:y_i}. As a result, during the backpropagations, instead of going through the one-hot represented scheduling, which will break the backpropagation chain, it goes through the differentiable Gumbel-Softmax approximations to train the class probabilities $\pi$, which will update the one-hot selections in the forward pass in the next iteration. Note that, in the forward pass of the framework, the scheduling is converted to one-hot representation to guarantee the correctness of the scheduling solutions at each iteration regarding its dependency. 

\subsubsection{Dependency Modeling}

To model the dependency between nodes during the scheduling, we proposed conditional Gumbel-Softmax, where we include the dependency distribution vector $D_{n}$ between the current node $n$ and its parent nodes in Equation~\ref{equ:y_i}. Being aware of the dependency, the available stages for scheduling of a child node should not be earlier than all its parents nodes. For example, in Figure~\ref{fig:case_study}, when node $1$ is scheduled at stage $1$, i.e., the stage selection of node $1$ is $S_{1} = [1, 0, 0]$, the available stages for its child nodes, i.e., node $3, 4$, are all the three stages $1$ and $2$ and $3$, i.e., the dependency distribution vector $D_{3/4}$ for node $3/4$ is $[1, 1, 1]$ with equal probabilities on all available stages. However, for node $5$, it has two parents node $4$ and node $2$. When the scheduling stage for node $4$ is stage 2, i.e., $S_{4} = [0, 1, 0]$, the available stages for its child node $5$ are stage $2$ and $3$, i.e., the $D_{5}$ from the dependency of node $4$ is $[0, 1, 1]$. As a result, for node $5$, with dependencies from both parents node $2$ and node $4$, its available stags are stage $2$ and $3$, i.e., $D_{5} = [0, 1, 1]$. The computation of the dependency vector $D$ can be realized by the \texttt{cumsum} of the one-hot represented stage selections of its parents in a differentiable way.

Then we multiply the dependency vector $D_{n}$ for each node on the approximation vector $y_{n}$ in Equation~\ref{equ:y_i} after Gumbel-Softmax to guarantee the available stages for node $n$ during the training process follow the dependencies from its parents, while keeping the differentiability in the framework.  

%\subsubsection{ScheduleNet framework}

% \begin{figure*}[!htb]
%     \centering
%     \includegraphics[width=1\linewidth]{icml2024/figs/framework_overview-crop.pdf}
%     \caption{The overview of the framework ScheduleNet. }
%     \label{fig:overview}
% \end{figure*}


%Given a DAG $G(V, E)$, where $V$ is the set of nodes and $E$ is the set of edges, and the expected stages (Latency) $L$, in the framework, the trainable parameters have a dimension of $|V|\times L$, where we formulate an $L-$dimensional vector for the stage selection for each node $n\in V$. Additionally, the combinatorial optimization of $|V|$ stage selections are constrained and connected by $|E|$ dependency vectors. In the framework, the forward pass goes through the network following the topological order of the network to guarantee that the child nodes are scheduled after their parent nodes.


 
 %This can significantly improve the solving performance and effectively utilize modern computing platforms such as GPUs and TPUs. While the CO problems can be solved using SGD, our proposed approach naturally offers stochastic intermediate results, and the solving efforts (runtime) can be fully controlled by the stochastic iterations.

% We explored two formulations for the ASAP loss function:

% \paragraph{{\color{red}Lifetime}} -- 
% \begin{equation}
%     Loss_{lifetime} = \Sigma_{i=1}^{|E|} e_{i}
%      \label{equ:loss_lifetime}
% \end{equation}
% where $e_{i}$ is the lifetime of an edge represented by the onehot solution generated for Node $u$ and Node $v$, noted as $S_u$, $S_v$. Then $e_{i} = sum{cumsum{S_u}-cumsum{S_v}}$.

% \paragraph{{\color{red}Lifetime entropy}} --
% \begin{equation}
%     Loss_{entropyLifetime} = -\Sigma_{i=1}^{|E|} \frac{e_{i}}{|E|*(L-1)}\text{log} \frac{e_{i}}{|E|*(L-1)}
%     \label{equ:loss_entropyLifetime}
% \end{equation}
% where $e{i}$ is the same formulation as in Equation \ref{equ:loss_lifetime}. With this formulation, we can minimize the new Entropy Loss with the lifetime of each edge as input to minimize the average lifetime of the edges.







==> icml2024/6-related_work.tex <==
%\section{Related Works}
%\label{sec:related_work}

==> icml2024/figs/results.tex <==
\begin{figure*}[htbp]
\centering

% Row 1
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_1.pdf}
    \caption{Random Workload 1}
\end{subfigure}
% \quad
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_2.pdf}
    \caption{Random Workload 2}
\end{subfigure}
% \quad
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_3.pdf}
    \caption{Random Workload 3}
\end{subfigure}

\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_4.pdf}
    \caption{Random Workload 4}
\end{subfigure}
% \quad
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_5.pdf}
    \caption{Random Workload 5}
\end{subfigure}
% \quad
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_6.pdf}
    \caption{Random Workload 6}
\end{subfigure}

\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_7.pdf}
    \caption{Random Workload 7}
\end{subfigure}
% \quad
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_8.pdf}
    \caption{Random Workload 8}
\end{subfigure}
% \quad
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_9.pdf}
    \caption{Random Workload 9}
\end{subfigure}

\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_10.pdf}
    \caption{Random Workload 10}
\end{subfigure}
% \quad
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_11.pdf}
    \caption{Random Workload 11}
\end{subfigure}
% \quad
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_12.pdf}
    \caption{Random Workload 12}
\end{subfigure}

\caption{Random graphs}
\label{fig:random_results}
\end{figure*}

\begin{figure*}[htbp]
\centering

\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_13.pdf}
    \caption{Adder}
\end{subfigure}
% \quad
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_19.pdf}
    \caption{Adder (M)}
\end{subfigure}
% \quad
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_14.pdf}
    \caption{Barrel shifter}
\end{subfigure}

\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_20.pdf}
    \caption{Barrel shifter (M)}
\end{subfigure}
% \quad
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_15.pdf}
    \caption{i2c controller}
\end{subfigure}
% \quad
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_21.pdf}
    \caption{i2c controller (M)}
\end{subfigure}

\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_16.pdf}
    \caption{Max}
\end{subfigure}
% \quad
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_22.pdf}
    \caption{Max (M)}
\end{subfigure}
% \quad
\begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_17.pdf}
    \caption{Square}
\end{subfigure}

\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_23.pdf}
    \caption{Square (M)}
\end{subfigure}
% \quad
\begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_18.pdf}
    \caption{Voter}
\end{subfigure}
% \quad
\begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{icml2024/figs/results_figs/figure_24.pdf}
    \caption{Voter (M)}
\end{subfigure}

\caption{EPFL figs}
\label{fig:epft_figs}
\end{figure*}

==> tbls/compare_all.tex <==
\begin{table*}[t]
\centering
\caption{Comparison with all benchmarks: Random workload 1-3: Dense, with nodes up to 1000; Random workload 4-6: Sparse, with nodes up to 1000; Random workload 7-9: Sparse, with nodes up to 5000; Random workload 10-12: Sparse, with nodes up to 10000; (M): Technology mapping}
\label{tab:compare_all}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|ccccccccccc|}
\hline
\multirow{2}{*}{\textbf{Design}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{11}{c|}{\textbf{Running time and respective Objective Scheduling Progress}} \\ \cline{3-13} 
 &  & \multicolumn{1}{c|}{0 (s)} & \multicolumn{1}{c|}{360 (s)} & \multicolumn{1}{c|}{720 (s)} & \multicolumn{1}{c|}{1080 (s)} & \multicolumn{1}{c|}{1440 (s)} & \multicolumn{1}{c|}{1800 (s)} & \multicolumn{1}{c|}{2160 (s)} & \multicolumn{1}{c|}{2520 (s)} & \multicolumn{1}{c|}{2880 (s)} & \multicolumn{1}{c|}{3240 (s)} & 3600 (s) \\ \hline
\multirow{2}{*}{Random workload 1} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{98.20\%} & \multicolumn{1}{c|}{97.20\%} & \multicolumn{1}{c|}{\textbf{10.09\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \textbf{10.03\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{16.60\%}} & \multicolumn{1}{c|}{\textbf{16.60\%}} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{2}{*}{Random workload 2} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{99.29\%} & \multicolumn{1}{c|}{98.52\%} & \multicolumn{1}{c|}{\textbf{10.05\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.02\%}} & \textbf{10.02\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{18.97\%}} & \multicolumn{1}{c|}{\textbf{18.97\%}} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{2}{*}{Random workload 3} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{96.69\%} & \multicolumn{1}{c|}{26.72\%} & \multicolumn{1}{c|}{\textbf{10.05\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \textbf{10.04\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{17.57\%}} & \multicolumn{1}{c|}{\textbf{17.57\%}} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{2}{*}{Random workload 4} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.01\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{12.31\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{2}{*}{Random workload 5} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.01\%}} & \multicolumn{1}{c|}{\textbf{10.01\%}} & \multicolumn{1}{c|}{\textbf{10.01\%}} & \multicolumn{1}{c|}{\textbf{10.01\%}} & \multicolumn{1}{c|}{\textbf{10.01\%}} & \multicolumn{1}{c|}{\textbf{10.01\%}} & \multicolumn{1}{c|}{\textbf{10.01\%}} & \multicolumn{1}{c|}{\textbf{10.01\%}} & \multicolumn{1}{c|}{\textbf{10.01\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{12.38\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{2}{*}{Random workload 6} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{13.55\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{2}{*}{Random workload 7} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{83.23\%} & \multicolumn{1}{c|}{80.84\%} & \multicolumn{1}{c|}{25.20\%} & \multicolumn{1}{c|}{\textbf{10.01\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{13.74\%}} & \multicolumn{1}{c|}{\textbf{13.74\%}} & \multicolumn{1}{c|}{\textbf{13.74\%}} & \multicolumn{1}{c|}{13.74\%} & \multicolumn{1}{c|}{13.74\%} & \multicolumn{1}{c|}{13.74\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{2}{*}{Random workload 8} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{85.73\%} & \multicolumn{1}{c|}{82.35\%} & \multicolumn{1}{c|}{25.48\%} & \multicolumn{1}{c|}{\textbf{11.29\%}} & \multicolumn{1}{c|}{\textbf{10.01\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{15.00\%}} & \multicolumn{1}{c|}{\textbf{14.85\%}} & \multicolumn{1}{c|}{\textbf{14.49\%}} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & 14.49\% \\ \hline
\multirow{2}{*}{Random workload 9} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{86.94\%} & \multicolumn{1}{c|}{29.34\%} & \multicolumn{1}{c|}{24.44\%} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{15.21\%}} & \multicolumn{1}{c|}{\textbf{15.21\%}} & \multicolumn{1}{c|}{\textbf{13.38\%}} & \multicolumn{1}{c|}{13.38\%} & \multicolumn{1}{c|}{13.38\%} & \multicolumn{1}{c|}{13.38\%} & \multicolumn{1}{c|}{13.38\%} & \multicolumn{1}{c|}{13.38\%} & \multicolumn{1}{c|}{13.38\%} & 13.38\% \\ \hline
\multirow{2}{*}{Random workload 10} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{89.85\%} & \multicolumn{1}{c|}{84.67\%} & \multicolumn{1}{c|}{83.80\%} & \multicolumn{1}{c|}{82.58\%} & \multicolumn{1}{c|}{81.78\%} & \multicolumn{1}{c|}{81.78\%} & \multicolumn{1}{c|}{81.11\%} & \multicolumn{1}{c|}{81.11\%} & 18.11\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{14.06\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \textbf{13.98\%} \\ \hline
\multirow{2}{*}{Random workload 11} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{91.05\%} & \multicolumn{1}{c|}{85.70\%} & \multicolumn{1}{c|}{85.70\%} & \multicolumn{1}{c|}{84.21\%} & \multicolumn{1}{c|}{83.56\%} & \multicolumn{1}{c|}{83.41\%} & \multicolumn{1}{c|}{83.16\%} & \multicolumn{1}{c|}{82.26\%} & 82.26\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \textbf{13.88\%} \\ \hline
\multirow{2}{*}{Random workload 12} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{88.99\%} & \multicolumn{1}{c|}{85.96\%} & \multicolumn{1}{c|}{85.96\%} & \multicolumn{1}{c|}{85.89\%} & \multicolumn{1}{c|}{85.05\%} & \multicolumn{1}{c|}{84.00\%} & \multicolumn{1}{c|}{83.79\%} & \multicolumn{1}{c|}{82.80\%} & 82.80\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \textbf{13.94\%} \\ \hline
\multirow{2}{*}{Adder} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{14.90\%}} & \multicolumn{1}{c|}{\textbf{10.12\%}} & \multicolumn{1}{c|}{\textbf{10.10\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \textbf{10.08\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{17.00\%} & \multicolumn{1}{c|}{17.00\%} & \multicolumn{1}{c|}{17.00\%} & \multicolumn{1}{c|}{17.00\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{2}{*}{Barrel Shifter} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{13.12\%}} & \multicolumn{1}{c|}{\textbf{13.10\%}} & \textbf{13.07\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{25.19\%}} & \multicolumn{1}{c|}{\textbf{20.07\%}} & \multicolumn{1}{c|}{\textbf{20.07\%}} & \multicolumn{1}{c|}{\textbf{19.25\%}} & \multicolumn{1}{c|}{\textbf{19.25\%}} & \multicolumn{1}{c|}{\textbf{19.25\%}} & \multicolumn{1}{c|}{\textbf{19.25\%}} & \multicolumn{1}{c|}{19.25\%} & \multicolumn{1}{c|}{19.25\%} & 19.25\% \\ \hline
\multirow{2}{*}{i2c controller} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{97.43\%} & \multicolumn{1}{c|}{97.43\%} & \multicolumn{1}{c|}{97.43\%} & \multicolumn{1}{c|}{\textbf{10.92\%}} & \multicolumn{1}{c|}{\textbf{10.76\%}} & \multicolumn{1}{c|}{\textbf{10.70\%}} & \multicolumn{1}{c|}{\textbf{10.62\%}} & \multicolumn{1}{c|}{\textbf{10.59\%}} & \multicolumn{1}{c|}{\textbf{10.59\%}} & \textbf{10.59\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{15.45\%}} & \multicolumn{1}{c|}{\textbf{14.68\%}} & \multicolumn{1}{c|}{\textbf{14.68\%}} & \multicolumn{1}{c|}{14.68\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{2}{*}{Max} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{29.51\%} & \multicolumn{1}{c|}{27.41\%} & \multicolumn{1}{c|}{27.41\%} & \multicolumn{1}{c|}{27.16\%} & \multicolumn{1}{c|}{\textbf{18.32\%}} & \multicolumn{1}{c|}{\textbf{14.72\%}} & \multicolumn{1}{c|}{\textbf{12.90\%}} & \multicolumn{1}{c|}{\textbf{11.02\%}} & \textbf{10.83\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{38.22\%}} & \multicolumn{1}{c|}{\textbf{38.22\%}} & \multicolumn{1}{c|}{\textbf{38.43\%}} & \multicolumn{1}{c|}{\textbf{25.64\%}} & \multicolumn{1}{c|}{\textbf{25.18\%}} & \multicolumn{1}{c|}{25.18\%} & \multicolumn{1}{c|}{18.79\%} & \multicolumn{1}{c|}{18.79\%} & \multicolumn{1}{c|}{18.79\%} & 18.67\% \\ \hline
\multirow{2}{*}{Priority encoder} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.30\%}} & \multicolumn{1}{c|}{\textbf{10.28\%}} & \multicolumn{1}{c|}{\textbf{10.27\%}} & \multicolumn{1}{c|}{\textbf{10.22\%}} & \multicolumn{1}{c|}{\textbf{10.22\%}} & \multicolumn{1}{c|}{\textbf{10.22\%}} & \multicolumn{1}{c|}{\textbf{10.20\%}} & \multicolumn{1}{c|}{\textbf{10.20\%}} & \textbf{10.20\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{19.00\%}} & \multicolumn{1}{c|}{19.00\%} & \multicolumn{1}{c|}{19.00\%} & \multicolumn{1}{c|}{19.00\%} & \multicolumn{1}{c|}{18.44\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{2}{*}{Square} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{27.80\%}} & \multicolumn{1}{c|}{\textbf{27.80\%}} & \multicolumn{1}{c|}{\textbf{27.80\%}} & \multicolumn{1}{c|}{\textbf{27.80\%}} & \multicolumn{1}{c|}{\textbf{27.80\%}} & \multicolumn{1}{c|}{\textbf{27.10\%}} & \multicolumn{1}{c|}{\textbf{27.10\%}} & \multicolumn{1}{c|}{\textbf{23.39\%}} & \multicolumn{1}{c|}{\textbf{23.39\%}} & \textbf{23.39\%} \\ \hline
\multirow{2}{*}{Voter} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{22.56\%}} & \multicolumn{1}{c|}{\textbf{22.56\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \textbf{18.45\%} \\ \hline
\multirow{2}{*}{Adder (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.23\%}} & \multicolumn{1}{c|}{\textbf{10.11\%}} & \multicolumn{1}{c|}{\textbf{10.10\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.05\%}} & \multicolumn{1}{c|}{\textbf{10.05\%}} & \multicolumn{1}{c|}{\textbf{10.05\%}} & \textbf{10.05\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{13.86\%}} & \multicolumn{1}{c|}{\textbf{13.86\%}} & \multicolumn{1}{c|}{13.86\%} & \multicolumn{1}{c|}{13.86\%} & \multicolumn{1}{c|}{13.86\%} & \multicolumn{1}{c|}{13.36\%} & \multicolumn{1}{c|}{13.36\%} & \multicolumn{1}{c|}{13.36\%} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{2}{*}{Barrel Shifter (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{97.84\%} & \multicolumn{1}{c|}{97.82\%} & \multicolumn{1}{c|}{97.82\%} & \multicolumn{1}{c|}{97.82\%} & \multicolumn{1}{c|}{97.64\%} & \multicolumn{1}{c|}{97.64\%} & \multicolumn{1}{c|}{97.62\%} & \multicolumn{1}{c|}{\textbf{15.21\%}} & \textbf{12.68\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{21.99\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{20.15\%} & 20.15\% \\ \hline
\multirow{2}{*}{i2c controller (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{98.51\%} & \multicolumn{1}{c|}{\textbf{11.49\%}} & \multicolumn{1}{c|}{\textbf{10.66\%}} & \multicolumn{1}{c|}{\textbf{10.63\%}} & \multicolumn{1}{c|}{\textbf{10.57\%}} & \multicolumn{1}{c|}{\textbf{10.57\%}} & \multicolumn{1}{c|}{\textbf{10.57\%}} & \multicolumn{1}{c|}{\textbf{10.57\%}} & \multicolumn{1}{c|}{\textbf{10.57\%}} & \textbf{10.57\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{21.81\%}} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{2}{*}{Max (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{19.11\%}} & \multicolumn{1}{c|}{\textbf{19.11\%}} & \multicolumn{1}{c|}{\textbf{19.11\%}} & \multicolumn{1}{c|}{\textbf{19.11\%}} & \multicolumn{1}{c|}{\textbf{19.11\%}} & \multicolumn{1}{c|}{19.11\%} & \multicolumn{1}{c|}{19.11\%} & \multicolumn{1}{c|}{18.38\%} & \textbf{12.46\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{28.53\%}} & \multicolumn{1}{c|}{28.53\%} & \multicolumn{1}{c|}{28.53\%} & \multicolumn{1}{c|}{28.53\%} & \multicolumn{1}{c|}{24.49\%} & \multicolumn{1}{c|}{23.96\%} & \multicolumn{1}{c|}{\textbf{17.73\%}} & \multicolumn{1}{c|}{\textbf{17.75\%}} & \multicolumn{1}{c|}{\textbf{17.29\%}} & 16.04\% \\ \hline
\multirow{2}{*}{Priority encoder (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.22\%}} & \multicolumn{1}{c|}{\textbf{10.18\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \textbf{10.17\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{13.59\%} & \multicolumn{1}{c|}{13.39\%} & \multicolumn{1}{c|}{13.39\%} & \multicolumn{1}{c|}{13.39\%} & \multicolumn{1}{c|}{13.39\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{2}{*}{Square (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{20.50\%}} & \multicolumn{1}{c|}{\textbf{20.50\%}} & \multicolumn{1}{c|}{\textbf{20.50\%}} & \multicolumn{1}{c|}{\textbf{20.50\%}} & \multicolumn{1}{c|}{\textbf{20.50\%}} & \multicolumn{1}{c|}{\textbf{18.79\%}} & \multicolumn{1}{c|}{\textbf{18.79\%}} & \multicolumn{1}{c|}{\textbf{17.33\%}} & \multicolumn{1}{c|}{\textbf{17.33\%}} & \textbf{17.33\%} \\ \hline
\multirow{2}{*}{Voter (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{11.71\%}} & \multicolumn{1}{c|}{\textbf{11.71\%}} & \multicolumn{1}{c|}{\textbf{11.13\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \textbf{10.44\%} \\ \hline
\end{tabular}%
}
\end{table*}

==> tbls/compare_epfl.tex <==
\begin{table*}[t]
\centering
\caption{Comparison with EPFL benchmarks: (M): Technology mapping}
\label{tab:compare_epfl}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|ccccccccccc|}
\hline
\multirow{2}{*}{\textbf{Design}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{11}{c|}{\textbf{Running time and Respective Objective Scheduling Progress}} \\ \cline{3-13} 
 &  & \multicolumn{1}{c|}{0 (s)} & \multicolumn{1}{c|}{360 (s)} & \multicolumn{1}{c|}{720 (s)} & \multicolumn{1}{c|}{1080 (s)} & \multicolumn{1}{c|}{1440 (s)} & \multicolumn{1}{c|}{1800 (s)} & \multicolumn{1}{c|}{2160 (s)} & \multicolumn{1}{c|}{2520 (s)} & \multicolumn{1}{c|}{2880 (s)} & \multicolumn{1}{c|}{3240 (s)} & 3600 (s) \\ \hline
\multirow{3}{*}{Adder} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{14.90\%}} & \multicolumn{1}{c|}{\textbf{10.12\%}} & \multicolumn{1}{c|}{10.10\%} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \textbf{10.08\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{20.92\%} & \multicolumn{1}{c|}{10.17\%} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \textbf{10.08\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{17.00\%} & \multicolumn{1}{c|}{17.00\%} & \multicolumn{1}{c|}{17.00\%} & \multicolumn{1}{c|}{17.00\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Barrel shifter} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{13.12\%}} & \multicolumn{1}{c|}{\textbf{13.10\%}} & \textbf{13.07\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{69.55\%} & \multicolumn{1}{c|}{55.55\%} & \multicolumn{1}{c|}{55.55\%} & \multicolumn{1}{c|}{49.91\%} & \multicolumn{1}{c|}{49.91\%} & \multicolumn{1}{c|}{49.91\%} & \multicolumn{1}{c|}{49.91\%} & \multicolumn{1}{c|}{49.91\%} & \multicolumn{1}{c|}{49.91\%} & 49.91\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{25.19\%}} & \multicolumn{1}{c|}{\textbf{20.07\%}} & \multicolumn{1}{c|}{\textbf{20.07\%}} & \multicolumn{1}{c|}{\textbf{19.25\%}} & \multicolumn{1}{c|}{\textbf{19.25\%}} & \multicolumn{1}{c|}{\textbf{19.25\%}} & \multicolumn{1}{c|}{\textbf{19.25\%}} & \multicolumn{1}{c|}{19.25\%} & \multicolumn{1}{c|}{19.25\%} & 19.25\% \\ \hline
\multirow{3}{*}{i2c controller} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{97.43\%} & \multicolumn{1}{c|}{97.43\%} & \multicolumn{1}{c|}{97.43\%} & \multicolumn{1}{c|}{\textbf{10.92\%}} & \multicolumn{1}{c|}{\textbf{10.76\%}} & \multicolumn{1}{c|}{\textbf{10.70\%}} & \multicolumn{1}{c|}{\textbf{10.62\%}} & \multicolumn{1}{c|}{\textbf{10.59\%}} & \multicolumn{1}{c|}{\textbf{10.59\%}} & \textbf{10.59\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{25.14\%} & \multicolumn{1}{c|}{25.14\%} & \multicolumn{1}{c|}{25.14\%} & \multicolumn{1}{c|}{25.14\%} & \multicolumn{1}{c|}{25.14\%} & \multicolumn{1}{c|}{25.14\%} & \multicolumn{1}{c|}{25.14\%} & \multicolumn{1}{c|}{25.14\%} & 25.14\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{15.45\%}} & \multicolumn{1}{c|}{\textbf{14.68\%}} & \multicolumn{1}{c|}{\textbf{14.68\%}} & \multicolumn{1}{c|}{14.68\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Max} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{29.51\%} & \multicolumn{1}{c|}{27.41\%} & \multicolumn{1}{c|}{27.41\%} & \multicolumn{1}{c|}{27.16\%} & \multicolumn{1}{c|}{\textbf{18.32\%}} & \multicolumn{1}{c|}{\textbf{14.72\%}} & \multicolumn{1}{c|}{\textbf{12.90\%}} & \multicolumn{1}{c|}{\textbf{11.02\%}} & \textbf{10.83\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{38.84\%} & \multicolumn{1}{c|}{33.62\%} & \multicolumn{1}{c|}{33.62\%} & \multicolumn{1}{c|}{33.62\%} & \multicolumn{1}{c|}{33.62\%} & \multicolumn{1}{c|}{33.62\%} & \multicolumn{1}{c|}{33.62\%} & \multicolumn{1}{c|}{25.71\%} & 25.71\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{38.22\%}} & \multicolumn{1}{c|}{\textbf{38.22\%}} & \multicolumn{1}{c|}{\textbf{38.43\%}} & \multicolumn{1}{c|}{\textbf{25.64\%}} & \multicolumn{1}{c|}{\textbf{25.18\%}} & \multicolumn{1}{c|}{25.18\%} & \multicolumn{1}{c|}{18.79\%} & \multicolumn{1}{c|}{18.79\%} & \multicolumn{1}{c|}{18.79\%} & 18.67\% \\ \hline
\multirow{3}{*}{Priority encoder} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.30\%}} & \multicolumn{1}{c|}{\textbf{10.28\%}} & \multicolumn{1}{c|}{\textbf{10.27\%}} & \multicolumn{1}{c|}{\textbf{10.22\%}} & \multicolumn{1}{c|}{\textbf{10.22\%}} & \multicolumn{1}{c|}{\textbf{10.22\%}} & \multicolumn{1}{c|}{\textbf{10.20\%}} & \multicolumn{1}{c|}{\textbf{10.20\%}} & \textbf{10.20\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{55.82\%} & \multicolumn{1}{c|}{55.82\%} & \multicolumn{1}{c|}{24.19\%} & \multicolumn{1}{c|}{24.19\%} & \multicolumn{1}{c|}{15.41\%} & \multicolumn{1}{c|}{15.41\%} & \multicolumn{1}{c|}{15.41\%} & \multicolumn{1}{c|}{15.41\%} & \multicolumn{1}{c|}{11.45\%} & 11.45\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{19.00\%}} & \multicolumn{1}{c|}{19.00\%} & \multicolumn{1}{c|}{19.00\%} & \multicolumn{1}{c|}{19.00\%} & \multicolumn{1}{c|}{18.44\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Square} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{27.80\%}} & \multicolumn{1}{c|}{\textbf{27.80\%}} & \multicolumn{1}{c|}{\textbf{27.80\%}} & \multicolumn{1}{c|}{\textbf{27.80\%}} & \multicolumn{1}{c|}{\textbf{27.80\%}} & \multicolumn{1}{c|}{\textbf{27.10\%}} & \multicolumn{1}{c|}{\textbf{27.10\%}} & \multicolumn{1}{c|}{\textbf{23.39\%}} & \multicolumn{1}{c|}{\textbf{23.39\%}} & \textbf{23.39\%} \\ \hline
\multirow{3}{*}{Voter} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{22.56\%}} & \multicolumn{1}{c|}{\textbf{22.56\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \textbf{18.45\%} \\ \hline
\multirow{3}{*}{Adder (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.23\%}} & \multicolumn{1}{c|}{\textbf{10.11\%}} & \multicolumn{1}{c|}{\textbf{10.10\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.05\%}} & \multicolumn{1}{c|}{10.05\%} & \multicolumn{1}{c|}{10.05\%} & 10.05\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{35.97\%} & \multicolumn{1}{c|}{28.91\%} & \multicolumn{1}{c|}{28.91\%} & \multicolumn{1}{c|}{28.91\%} & \multicolumn{1}{c|}{28.91\%} & \multicolumn{1}{c|}{10.12\%} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \textbf{10.04\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{13.86\%}} & \multicolumn{1}{c|}{\textbf{13.86\%}} & \multicolumn{1}{c|}{13.86\%} & \multicolumn{1}{c|}{13.86\%} & \multicolumn{1}{c|}{13.86\%} & \multicolumn{1}{c|}{13.36\%} & \multicolumn{1}{c|}{13.36\%} & \multicolumn{1}{c|}{13.36\%} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Barrel shifter (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{97.84\%} & \multicolumn{1}{c|}{97.82\%} & \multicolumn{1}{c|}{97.82\%} & \multicolumn{1}{c|}{97.82\%} & \multicolumn{1}{c|}{97.64\%} & \multicolumn{1}{c|}{97.64\%} & \multicolumn{1}{c|}{97.62\%} & \multicolumn{1}{c|}{\textbf{15.21\%}} & \textbf{12.68\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{80.46\%} & 80.46\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{21.99\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{20.15\%} & 20.15\% \\ \hline
\multirow{3}{*}{i2c controller (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{98.51\%} & \multicolumn{1}{c|}{\textbf{11.49\%}} & \multicolumn{1}{c|}{\textbf{10.66\%}} & \multicolumn{1}{c|}{\textbf{10.63\%}} & \multicolumn{1}{c|}{\textbf{10.57\%}} & \multicolumn{1}{c|}{\textbf{10.57\%}} & \multicolumn{1}{c|}{\textbf{10.57\%}} & \multicolumn{1}{c|}{\textbf{10.57\%}} & \multicolumn{1}{c|}{\textbf{10.57\%}} & \textbf{10.57\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{12.87\%}} & \multicolumn{1}{c|}{12.87\%} & \multicolumn{1}{c|}{12.87\%} & \multicolumn{1}{c|}{12.87\%} & \multicolumn{1}{c|}{12.87\%} & \multicolumn{1}{c|}{12.87\%} & \multicolumn{1}{c|}{12.08\%} & \multicolumn{1}{c|}{12.08\%} & \multicolumn{1}{c|}{12.08\%} & 12.08\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{21.81\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Max (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{19.11\%}} & \multicolumn{1}{c|}{\textbf{19.11\%}} & \multicolumn{1}{c|}{\textbf{19.11\%}} & \multicolumn{1}{c|}{\textbf{19.11\%}} & \multicolumn{1}{c|}{\textbf{19.11\%}} & \multicolumn{1}{c|}{19.11\%} & \multicolumn{1}{c|}{19.11\%} & \multicolumn{1}{c|}{18.38\%} & \textbf{12.46\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{71.07\%} & \multicolumn{1}{c|}{57.39\%} & \multicolumn{1}{c|}{57.39\%} & \multicolumn{1}{c|}{57.39\%} & \multicolumn{1}{c|}{57.39\%} & \multicolumn{1}{c|}{57.39\%} & \multicolumn{1}{c|}{57.39\%} & \multicolumn{1}{c|}{57.39\%} & 57.39\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{28.53\%}} & \multicolumn{1}{c|}{28.53\%} & \multicolumn{1}{c|}{28.53\%} & \multicolumn{1}{c|}{28.53\%} & \multicolumn{1}{c|}{24.49\%} & \multicolumn{1}{c|}{23.96\%} & \multicolumn{1}{c|}{\textbf{17.73\%}} & \multicolumn{1}{c|}{\textbf{17.75\%}} & \multicolumn{1}{c|}{\textbf{17.29\%}} & 16.04\% \\ \hline
\multirow{3}{*}{Priority encoder (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.22\%}} & \multicolumn{1}{c|}{\textbf{10.18\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \textbf{10.17\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{28.68\%} & \multicolumn{1}{c|}{23.13\%} & \multicolumn{1}{c|}{18.66\%} & \multicolumn{1}{c|}{16.82\%} & \multicolumn{1}{c|}{14.35\%} & \multicolumn{1}{c|}{10.31\%} & \multicolumn{1}{c|}{10.23\%} & \multicolumn{1}{c|}{10.23\%} & \multicolumn{1}{c|}{10.21\%} & 10.21\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{13.59\%} & \multicolumn{1}{c|}{13.39\%} & \multicolumn{1}{c|}{13.39\%} & \multicolumn{1}{c|}{13.39\%} & \multicolumn{1}{c|}{13.39\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Square (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{20.50\%}} & \multicolumn{1}{c|}{\textbf{20.50\%}} & \multicolumn{1}{c|}{\textbf{20.50\%}} & \multicolumn{1}{c|}{\textbf{20.50\%}} & \multicolumn{1}{c|}{\textbf{20.50\%}} & \multicolumn{1}{c|}{\textbf{18.79\%}} & \multicolumn{1}{c|}{\textbf{18.79\%}} & \multicolumn{1}{c|}{\textbf{17.33\%}} & \multicolumn{1}{c|}{\textbf{17.33\%}} & \textbf{17.33\%} \\ \hline
\multirow{3}{*}{Voter (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{11.71\%}} & \multicolumn{1}{c|}{\textbf{11.71\%}} & \multicolumn{1}{c|}{\textbf{11.13\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \textbf{10.44\%} \\ \hline
\end{tabular}%
}
\end{table*}

==> tbls/compare_gurobi_all.tex <==
\begin{table*}[t]
\centering
\caption{
% Comparison with all benchmarks: Random workload 1-3: Dense, with nodes up to 1000; Random workload 4-6: Sparse, with nodes up to 1000; Random workload 7-9: Sparse, with nodes up to 5000; Random workload 10-12: Sparse, with nodes up to 10000; (M): Technology mapping
}
\label{tab:compare_all_gurobi}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|ccccccccccc|}
\hline
\multirow{2}{*}{\textbf{Design}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{11}{c|}{\textbf{Running time and respective Objective Scheduling Progress}} \\ \cline{3-13} 
 &  & \multicolumn{1}{c|}{0 (s)} & \multicolumn{1}{c|}{360 (s)} & \multicolumn{1}{c|}{720 (s)} & \multicolumn{1}{c|}{1080 (s)} & \multicolumn{1}{c|}{1440 (s)} & \multicolumn{1}{c|}{1800 (s)} & \multicolumn{1}{c|}{2160 (s)} & \multicolumn{1}{c|}{2520 (s)} & \multicolumn{1}{c|}{2880 (s)} & \multicolumn{1}{c|}{3240 (s)} & 3600 (s) \\ \hline
\multirow{3}{*}{Random workload 1} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{98.20\%} & \multicolumn{1}{c|}{97.20\%} & \multicolumn{1}{c|}{\textbf{10.09\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{10.03\%} & \multicolumn{1}{c|}{10.03\%} & \multicolumn{1}{c|}{10.03\%} & \multicolumn{1}{c|}{10.03\%} & 10.03\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{38.23\%} & \multicolumn{1}{c|}{32.19\%} & \multicolumn{1}{c|}{20.88\%} & \multicolumn{1}{c|}{10.12\%} & \multicolumn{1}{c|}{\textbf{10.02\%}} & \multicolumn{1}{c|}{\textbf{10.02\%}} & \multicolumn{1}{c|}{\textbf{10.02\%}} & \multicolumn{1}{c|}{\textbf{10.02\%}} & \textbf{10.02\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{16.60\%}} & \multicolumn{1}{c|}{\textbf{16.60\%}} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Random workload 2} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{99.29\%} & \multicolumn{1}{c|}{98.52\%} & \multicolumn{1}{c|}{\textbf{10.05\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.02\%}} & \textbf{10.02\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{57.84\%} & \multicolumn{1}{c|}{45.04\%} & \multicolumn{1}{c|}{38.84\%} & \multicolumn{1}{c|}{17.83\%} & \multicolumn{1}{c|}{17.83\%} & \multicolumn{1}{c|}{11.91\%} & \multicolumn{1}{c|}{10.96\%} & \multicolumn{1}{c|}{10.70\%} & 10.08\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{18.97\%}} & \multicolumn{1}{c|}{\textbf{18.97\%}} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Random workload 3} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{96.69\%} & \multicolumn{1}{c|}{26.72\%} & \multicolumn{1}{c|}{\textbf{10.05\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \textbf{10.04\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{47.01\%} & \multicolumn{1}{c|}{39.62\%} & \multicolumn{1}{c|}{17.75\%} & \multicolumn{1}{c|}{17.75\%} & \multicolumn{1}{c|}{11.03\%} & \multicolumn{1}{c|}{10.56\%} & \multicolumn{1}{c|}{10.49\%} & \multicolumn{1}{c|}{10.49\%} & 10.49\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{17.57\%}} & \multicolumn{1}{c|}{\textbf{17.57\%}} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Random workload 4} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{12.31\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Random workload 5} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{10.01\%} & \textbf{10.00\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{12.38\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Random workload 6} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{13.55\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Random workload 7} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{83.23\%} & \multicolumn{1}{c|}{80.84\%} & \multicolumn{1}{c|}{25.20\%} & \multicolumn{1}{c|}{\textbf{10.01\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{22.71\%} & \multicolumn{1}{c|}{10.51\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{13.74\%}} & \multicolumn{1}{c|}{\textbf{13.74\%}} & \multicolumn{1}{c|}{\textbf{13.74\%}} & \multicolumn{1}{c|}{13.74\%} & \multicolumn{1}{c|}{13.74\%} & \multicolumn{1}{c|}{13.74\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Random workload 8} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{85.73\%} & \multicolumn{1}{c|}{82.35\%} & \multicolumn{1}{c|}{25.48\%} & \multicolumn{1}{c|}{11.29\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{32.48\%} & \multicolumn{1}{c|}{\textbf{12.89\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{15.00\%}} & \multicolumn{1}{c|}{\textbf{14.85\%}} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & 14.49\% \\ \hline
\multirow{3}{*}{Random workload 9} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{86.94\%} & \multicolumn{1}{c|}{29.34\%} & \multicolumn{1}{c|}{24.44\%} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{24.08\%} & \multicolumn{1}{c|}{16.02\%} & \multicolumn{1}{c|}{15.96\%} & \multicolumn{1}{c|}{14.66\%} & \multicolumn{1}{c|}{14.66\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{15.21\%}} & \multicolumn{1}{c|}{\textbf{15.21\%}} & \multicolumn{1}{c|}{\textbf{13.38\%}} & \multicolumn{1}{c|}{13.38\%} & \multicolumn{1}{c|}{13.38\%} & \multicolumn{1}{c|}{13.38\%} & \multicolumn{1}{c|}{13.38\%} & \multicolumn{1}{c|}{13.38\%} & \multicolumn{1}{c|}{13.38\%} & 13.38\% \\ \hline
\multirow{3}{*}{Random workload 10} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{89.85\%} & \multicolumn{1}{c|}{84.67\%} & \multicolumn{1}{c|}{83.80\%} & \multicolumn{1}{c|}{82.58\%} & \multicolumn{1}{c|}{81.78\%} & \multicolumn{1}{c|}{81.78\%} & \multicolumn{1}{c|}{81.11\%} & \multicolumn{1}{c|}{81.11\%} & 18.11\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{29.37\%} & \multicolumn{1}{c|}{19.58\%} & \multicolumn{1}{c|}{19.57\%} & \multicolumn{1}{c|}{19.57\%} & \multicolumn{1}{c|}{16.77\%} & \multicolumn{1}{c|}{16.78\%} & \multicolumn{1}{c|}{16.77\%} & \multicolumn{1}{c|}{16.07\%} & 16.07\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{14.06\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \textbf{13.98\%} \\ \hline
\multirow{3}{*}{Random workload 11} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{91.05\%} & \multicolumn{1}{c|}{85.70\%} & \multicolumn{1}{c|}{85.70\%} & \multicolumn{1}{c|}{84.21\%} & \multicolumn{1}{c|}{83.56\%} & \multicolumn{1}{c|}{83.41\%} & \multicolumn{1}{c|}{83.16\%} & \multicolumn{1}{c|}{82.26\%} & 82.26\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{37.60\%} & \multicolumn{1}{c|}{16.12\%} & \multicolumn{1}{c|}{16.12\%} & \multicolumn{1}{c|}{15.93\%} & \multicolumn{1}{c|}{15.93\%} & \multicolumn{1}{c|}{\textbf{13.12\%}} & \multicolumn{1}{c|}{\textbf{13.10\%}} & \textbf{13.10\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{13.88\%} & \multicolumn{1}{c|}{13.88\%} & 13.88\% \\ \hline
\multirow{3}{*}{Random workload 12} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{88.99\%} & \multicolumn{1}{c|}{85.96\%} & \multicolumn{1}{c|}{85.96\%} & \multicolumn{1}{c|}{85.89\%} & \multicolumn{1}{c|}{85.05\%} & \multicolumn{1}{c|}{84.00\%} & \multicolumn{1}{c|}{83.79\%} & \multicolumn{1}{c|}{82.80\%} & 82.80\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{37.11\%} & \multicolumn{1}{c|}{20.44\%} & \multicolumn{1}{c|}{20.32\%} & \multicolumn{1}{c|}{20.26\%} & \multicolumn{1}{c|}{20.26\%} & \multicolumn{1}{c|}{\textbf{10.23\%}} & \multicolumn{1}{c|}{\textbf{10.23\%}} & \multicolumn{1}{c|}{\textbf{10.23\%}} & \textbf{10.23\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{13.94\%} & \multicolumn{1}{c|}{13.94\%} & \multicolumn{1}{c|}{13.94\%} & 13.94\% \\ \hline
\multirow{3}{*}{Adder} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{14.90\%}} & \multicolumn{1}{c|}{\textbf{10.12\%}} & \multicolumn{1}{c|}{10.10\%} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \textbf{10.08\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{20.92\%} & \multicolumn{1}{c|}{10.17\%} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \textbf{10.08\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{17.00\%} & \multicolumn{1}{c|}{17.00\%} & \multicolumn{1}{c|}{17.00\%} & \multicolumn{1}{c|}{17.00\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Barrel Shifter} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{13.12\%}} & \multicolumn{1}{c|}{\textbf{13.10\%}} & \textbf{13.07\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{69.55\%} & \multicolumn{1}{c|}{55.55\%} & \multicolumn{1}{c|}{55.55\%} & \multicolumn{1}{c|}{49.91\%} & \multicolumn{1}{c|}{49.91\%} & \multicolumn{1}{c|}{49.91\%} & \multicolumn{1}{c|}{49.91\%} & \multicolumn{1}{c|}{49.91\%} & \multicolumn{1}{c|}{49.91\%} & 49.91\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{25.19\%}} & \multicolumn{1}{c|}{\textbf{20.07\%}} & \multicolumn{1}{c|}{\textbf{20.07\%}} & \multicolumn{1}{c|}{\textbf{19.25\%}} & \multicolumn{1}{c|}{\textbf{19.25\%}} & \multicolumn{1}{c|}{\textbf{19.25\%}} & \multicolumn{1}{c|}{\textbf{19.25\%}} & \multicolumn{1}{c|}{19.25\%} & \multicolumn{1}{c|}{19.25\%} & 19.25\% \\ \hline
\multirow{3}{*}{i2c controller} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{97.43\%} & \multicolumn{1}{c|}{97.43\%} & \multicolumn{1}{c|}{97.43\%} & \multicolumn{1}{c|}{\textbf{10.92\%}} & \multicolumn{1}{c|}{\textbf{10.76\%}} & \multicolumn{1}{c|}{\textbf{10.70\%}} & \multicolumn{1}{c|}{\textbf{10.62\%}} & \multicolumn{1}{c|}{\textbf{10.59\%}} & \multicolumn{1}{c|}{\textbf{10.59\%}} & \textbf{10.59\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{25.14\%} & \multicolumn{1}{c|}{25.14\%} & \multicolumn{1}{c|}{25.14\%} & \multicolumn{1}{c|}{25.14\%} & \multicolumn{1}{c|}{25.14\%} & \multicolumn{1}{c|}{25.14\%} & \multicolumn{1}{c|}{25.14\%} & \multicolumn{1}{c|}{25.14\%} & 25.14\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{15.45\%}} & \multicolumn{1}{c|}{\textbf{14.68\%}} & \multicolumn{1}{c|}{\textbf{14.68\%}} & \multicolumn{1}{c|}{14.68\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Max} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{29.51\%} & \multicolumn{1}{c|}{27.41\%} & \multicolumn{1}{c|}{27.41\%} & \multicolumn{1}{c|}{27.16\%} & \multicolumn{1}{c|}{\textbf{18.32\%}} & \multicolumn{1}{c|}{\textbf{14.72\%}} & \multicolumn{1}{c|}{\textbf{12.90\%}} & \multicolumn{1}{c|}{\textbf{11.02\%}} & \textbf{10.83\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{38.84\%} & \multicolumn{1}{c|}{33.62\%} & \multicolumn{1}{c|}{33.62\%} & \multicolumn{1}{c|}{33.62\%} & \multicolumn{1}{c|}{33.62\%} & \multicolumn{1}{c|}{33.62\%} & \multicolumn{1}{c|}{33.62\%} & \multicolumn{1}{c|}{25.71\%} & 25.71\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{38.22\%}} & \multicolumn{1}{c|}{\textbf{38.22\%}} & \multicolumn{1}{c|}{\textbf{38.43\%}} & \multicolumn{1}{c|}{\textbf{25.64\%}} & \multicolumn{1}{c|}{\textbf{25.18\%}} & \multicolumn{1}{c|}{25.18\%} & \multicolumn{1}{c|}{18.79\%} & \multicolumn{1}{c|}{18.79\%} & \multicolumn{1}{c|}{18.79\%} & 18.67\% \\ \hline
\multirow{3}{*}{Priority encoder} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.30\%}} & \multicolumn{1}{c|}{\textbf{10.28\%}} & \multicolumn{1}{c|}{\textbf{10.27\%}} & \multicolumn{1}{c|}{\textbf{10.22\%}} & \multicolumn{1}{c|}{\textbf{10.22\%}} & \multicolumn{1}{c|}{\textbf{10.22\%}} & \multicolumn{1}{c|}{\textbf{10.20\%}} & \multicolumn{1}{c|}{\textbf{10.20\%}} & \textbf{10.20\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{55.82\%} & \multicolumn{1}{c|}{55.82\%} & \multicolumn{1}{c|}{24.19\%} & \multicolumn{1}{c|}{24.19\%} & \multicolumn{1}{c|}{15.41\%} & \multicolumn{1}{c|}{15.41\%} & \multicolumn{1}{c|}{15.41\%} & \multicolumn{1}{c|}{15.41\%} & \multicolumn{1}{c|}{11.45\%} & 11.45\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{19.00\%}} & \multicolumn{1}{c|}{19.00\%} & \multicolumn{1}{c|}{19.00\%} & \multicolumn{1}{c|}{19.00\%} & \multicolumn{1}{c|}{18.44\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Square} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{27.80\%}} & \multicolumn{1}{c|}{\textbf{27.80\%}} & \multicolumn{1}{c|}{\textbf{27.80\%}} & \multicolumn{1}{c|}{\textbf{27.80\%}} & \multicolumn{1}{c|}{\textbf{27.80\%}} & \multicolumn{1}{c|}{\textbf{27.10\%}} & \multicolumn{1}{c|}{\textbf{27.10\%}} & \multicolumn{1}{c|}{\textbf{23.39\%}} & \multicolumn{1}{c|}{\textbf{23.39\%}} & \textbf{23.39\%} \\ \hline
\multirow{3}{*}{Voter} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{22.56\%}} & \multicolumn{1}{c|}{\textbf{22.56\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \multicolumn{1}{c|}{\textbf{18.45\%}} & \textbf{18.45\%} \\ \hline
\multirow{3}{*}{Adder (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.23\%}} & \multicolumn{1}{c|}{\textbf{10.11\%}} & \multicolumn{1}{c|}{\textbf{10.10\%}} & \multicolumn{1}{c|}{\textbf{10.08\%}} & \multicolumn{1}{c|}{\textbf{10.05\%}} & \multicolumn{1}{c|}{10.05\%} & \multicolumn{1}{c|}{10.05\%} & 10.05\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{35.97\%} & \multicolumn{1}{c|}{28.91\%} & \multicolumn{1}{c|}{28.91\%} & \multicolumn{1}{c|}{28.91\%} & \multicolumn{1}{c|}{28.91\%} & \multicolumn{1}{c|}{10.12\%} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \textbf{10.04\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{13.86\%}} & \multicolumn{1}{c|}{\textbf{13.86\%}} & \multicolumn{1}{c|}{13.86\%} & \multicolumn{1}{c|}{13.86\%} & \multicolumn{1}{c|}{13.86\%} & \multicolumn{1}{c|}{13.36\%} & \multicolumn{1}{c|}{13.36\%} & \multicolumn{1}{c|}{13.36\%} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Barrel Shifter (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{97.84\%} & \multicolumn{1}{c|}{97.82\%} & \multicolumn{1}{c|}{97.82\%} & \multicolumn{1}{c|}{97.82\%} & \multicolumn{1}{c|}{97.64\%} & \multicolumn{1}{c|}{97.64\%} & \multicolumn{1}{c|}{97.62\%} & \multicolumn{1}{c|}{\textbf{15.21\%}} & \textbf{12.68\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{80.46\%} & 80.46\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{21.99\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{\textbf{20.15\%}} & \multicolumn{1}{c|}{20.15\%} & 20.15\% \\ \hline
\multirow{3}{*}{i2c controller (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{98.51\%} & \multicolumn{1}{c|}{\textbf{11.49\%}} & \multicolumn{1}{c|}{\textbf{10.66\%}} & \multicolumn{1}{c|}{\textbf{10.63\%}} & \multicolumn{1}{c|}{\textbf{10.57\%}} & \multicolumn{1}{c|}{\textbf{10.57\%}} & \multicolumn{1}{c|}{\textbf{10.57\%}} & \multicolumn{1}{c|}{\textbf{10.57\%}} & \multicolumn{1}{c|}{\textbf{10.57\%}} & \textbf{10.57\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{12.87\%}} & \multicolumn{1}{c|}{12.87\%} & \multicolumn{1}{c|}{12.87\%} & \multicolumn{1}{c|}{12.87\%} & \multicolumn{1}{c|}{12.87\%} & \multicolumn{1}{c|}{12.87\%} & \multicolumn{1}{c|}{12.08\%} & \multicolumn{1}{c|}{12.08\%} & \multicolumn{1}{c|}{12.08\%} & 12.08\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{21.81\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{18.34\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Max (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{19.11\%}} & \multicolumn{1}{c|}{\textbf{19.11\%}} & \multicolumn{1}{c|}{\textbf{19.11\%}} & \multicolumn{1}{c|}{\textbf{19.11\%}} & \multicolumn{1}{c|}{\textbf{19.11\%}} & \multicolumn{1}{c|}{19.11\%} & \multicolumn{1}{c|}{19.11\%} & \multicolumn{1}{c|}{18.38\%} & \textbf{12.46\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{71.07\%} & \multicolumn{1}{c|}{57.39\%} & \multicolumn{1}{c|}{57.39\%} & \multicolumn{1}{c|}{57.39\%} & \multicolumn{1}{c|}{57.39\%} & \multicolumn{1}{c|}{57.39\%} & \multicolumn{1}{c|}{57.39\%} & \multicolumn{1}{c|}{57.39\%} & 57.39\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{28.53\%}} & \multicolumn{1}{c|}{28.53\%} & \multicolumn{1}{c|}{28.53\%} & \multicolumn{1}{c|}{28.53\%} & \multicolumn{1}{c|}{24.49\%} & \multicolumn{1}{c|}{23.96\%} & \multicolumn{1}{c|}{\textbf{17.73\%}} & \multicolumn{1}{c|}{\textbf{17.75\%}} & \multicolumn{1}{c|}{\textbf{17.29\%}} & 16.04\% \\ \hline
\multirow{3}{*}{Priority encoder (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.22\%}} & \multicolumn{1}{c|}{\textbf{10.18\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \multicolumn{1}{c|}{\textbf{10.17\%}} & \textbf{10.17\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{28.68\%} & \multicolumn{1}{c|}{23.13\%} & \multicolumn{1}{c|}{18.66\%} & \multicolumn{1}{c|}{16.82\%} & \multicolumn{1}{c|}{14.35\%} & \multicolumn{1}{c|}{10.31\%} & \multicolumn{1}{c|}{10.23\%} & \multicolumn{1}{c|}{10.23\%} & \multicolumn{1}{c|}{10.21\%} & 10.21\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{13.59\%} & \multicolumn{1}{c|}{13.39\%} & \multicolumn{1}{c|}{13.39\%} & \multicolumn{1}{c|}{13.39\%} & \multicolumn{1}{c|}{13.39\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Square (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{20.50\%}} & \multicolumn{1}{c|}{\textbf{20.50\%}} & \multicolumn{1}{c|}{\textbf{20.50\%}} & \multicolumn{1}{c|}{\textbf{20.50\%}} & \multicolumn{1}{c|}{\textbf{20.50\%}} & \multicolumn{1}{c|}{\textbf{18.79\%}} & \multicolumn{1}{c|}{\textbf{18.79\%}} & \multicolumn{1}{c|}{\textbf{17.33\%}} & \multicolumn{1}{c|}{\textbf{17.33\%}} & \textbf{17.33\%} \\ \hline
\multirow{3}{*}{Voter (M)} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & 100.00\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{11.71\%}} & \multicolumn{1}{c|}{\textbf{11.71\%}} & \multicolumn{1}{c|}{\textbf{11.13\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \multicolumn{1}{c|}{\textbf{10.44\%}} & \textbf{10.44\%} \\ \hline
\end{tabular}%
}
\end{table*}

==> tbls/compare_random.tex <==
\begin{table*}[t]
\centering
\caption{Comparison with Random workload benchmarks: Random workload 1-3: Dense, with nodes up to 1000; Random workload 4-6: Sparse, with nodes up to 1000; Random workload 7-9: Sparse, with nodes up to 5000; Random workload 10-12: Sparse, with nodes up to 10000;}
\label{tab:compare_all_random}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|ccccccccccc|}
\hline
\multirow{2}{*}{\textbf{Design}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{11}{c|}{\textbf{Running time and Respective Objective Scheduling Progress}} \\ \cline{3-13} 
 &  & \multicolumn{1}{c|}{0 (s)} & \multicolumn{1}{c|}{360 (s)} & \multicolumn{1}{c|}{720 (s)} & \multicolumn{1}{c|}{1080 (s)} & \multicolumn{1}{c|}{1440 (s)} & \multicolumn{1}{c|}{1800 (s)} & \multicolumn{1}{c|}{2160 (s)} & \multicolumn{1}{c|}{2520 (s)} & \multicolumn{1}{c|}{2880 (s)} & \multicolumn{1}{c|}{3240 (s)} & 3600 (s) \\ \hline
\multirow{3}{*}{Random workload 1} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{98.20\%} & \multicolumn{1}{c|}{97.20\%} & \multicolumn{1}{c|}{\textbf{10.09\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{10.03\%} & \multicolumn{1}{c|}{10.03\%} & \multicolumn{1}{c|}{10.03\%} & \multicolumn{1}{c|}{10.03\%} & 10.03\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{38.23\%} & \multicolumn{1}{c|}{32.19\%} & \multicolumn{1}{c|}{20.88\%} & \multicolumn{1}{c|}{10.12\%} & \multicolumn{1}{c|}{\textbf{10.02\%}} & \multicolumn{1}{c|}{\textbf{10.02\%}} & \multicolumn{1}{c|}{\textbf{10.02\%}} & \multicolumn{1}{c|}{\textbf{10.02\%}} & \textbf{10.02\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{16.60\%}} & \multicolumn{1}{c|}{\textbf{16.60\%}} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Random workload 2} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{99.29\%} & \multicolumn{1}{c|}{98.52\%} & \multicolumn{1}{c|}{\textbf{10.05\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.03\%}} & \multicolumn{1}{c|}{\textbf{10.02\%}} & \textbf{10.02\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{57.84\%} & \multicolumn{1}{c|}{45.04\%} & \multicolumn{1}{c|}{38.84\%} & \multicolumn{1}{c|}{17.83\%} & \multicolumn{1}{c|}{17.83\%} & \multicolumn{1}{c|}{11.91\%} & \multicolumn{1}{c|}{10.96\%} & \multicolumn{1}{c|}{10.70\%} & 10.08\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{18.97\%}} & \multicolumn{1}{c|}{\textbf{18.97\%}} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Random workload 3} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{96.69\%} & \multicolumn{1}{c|}{26.72\%} & \multicolumn{1}{c|}{\textbf{10.05\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \textbf{10.04\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{47.01\%} & \multicolumn{1}{c|}{39.62\%} & \multicolumn{1}{c|}{17.75\%} & \multicolumn{1}{c|}{17.75\%} & \multicolumn{1}{c|}{11.03\%} & \multicolumn{1}{c|}{10.56\%} & \multicolumn{1}{c|}{10.49\%} & \multicolumn{1}{c|}{10.49\%} & 10.49\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{17.57\%}} & \multicolumn{1}{c|}{\textbf{17.57\%}} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Random workload 4} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{12.31\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Random workload 5} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{10.01\%} & \textbf{10.00\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{12.38\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Random workload 6} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{13.55\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Random workload 7} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{83.23\%} & \multicolumn{1}{c|}{80.84\%} & \multicolumn{1}{c|}{25.20\%} & \multicolumn{1}{c|}{\textbf{10.01\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{22.71\%} & \multicolumn{1}{c|}{10.51\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{13.74\%}} & \multicolumn{1}{c|}{\textbf{13.74\%}} & \multicolumn{1}{c|}{\textbf{13.74\%}} & \multicolumn{1}{c|}{13.74\%} & \multicolumn{1}{c|}{13.74\%} & \multicolumn{1}{c|}{13.74\%} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{Random workload 8} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{85.73\%} & \multicolumn{1}{c|}{82.35\%} & \multicolumn{1}{c|}{25.48\%} & \multicolumn{1}{c|}{11.29\%} & \multicolumn{1}{c|}{10.01\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{32.48\%} & \multicolumn{1}{c|}{\textbf{12.89\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{15.00\%}} & \multicolumn{1}{c|}{\textbf{14.85\%}} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & \multicolumn{1}{c|}{14.49\%} & 14.49\% \\ \hline
\multirow{3}{*}{Random workload 9} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{86.94\%} & \multicolumn{1}{c|}{29.34\%} & \multicolumn{1}{c|}{24.44\%} & \multicolumn{1}{c|}{\textbf{10.04\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{24.08\%} & \multicolumn{1}{c|}{16.02\%} & \multicolumn{1}{c|}{15.96\%} & \multicolumn{1}{c|}{14.66\%} & \multicolumn{1}{c|}{14.66\%} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \multicolumn{1}{c|}{\textbf{10.00\%}} & \textbf{10.00\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{15.21\%}} & \multicolumn{1}{c|}{\textbf{15.21\%}} & \multicolumn{1}{c|}{\textbf{13.38\%}} & \multicolumn{1}{c|}{13.38\%} & \multicolumn{1}{c|}{13.38\%} & \multicolumn{1}{c|}{13.38\%} & \multicolumn{1}{c|}{13.38\%} & \multicolumn{1}{c|}{13.38\%} & \multicolumn{1}{c|}{13.38\%} & 13.38\% \\ \hline
\multirow{3}{*}{Random workload 10} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{89.85\%} & \multicolumn{1}{c|}{84.67\%} & \multicolumn{1}{c|}{83.80\%} & \multicolumn{1}{c|}{82.58\%} & \multicolumn{1}{c|}{81.78\%} & \multicolumn{1}{c|}{81.78\%} & \multicolumn{1}{c|}{81.11\%} & \multicolumn{1}{c|}{81.11\%} & 18.11\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{29.37\%} & \multicolumn{1}{c|}{19.58\%} & \multicolumn{1}{c|}{19.57\%} & \multicolumn{1}{c|}{19.57\%} & \multicolumn{1}{c|}{16.77\%} & \multicolumn{1}{c|}{16.78\%} & \multicolumn{1}{c|}{16.77\%} & \multicolumn{1}{c|}{16.07\%} & 16.07\% \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{14.06\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \multicolumn{1}{c|}{\textbf{13.98\%}} & \textbf{13.98\%} \\ \hline
\multirow{3}{*}{Random workload 11} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{91.05\%} & \multicolumn{1}{c|}{85.70\%} & \multicolumn{1}{c|}{85.70\%} & \multicolumn{1}{c|}{84.21\%} & \multicolumn{1}{c|}{83.56\%} & \multicolumn{1}{c|}{83.41\%} & \multicolumn{1}{c|}{83.16\%} & \multicolumn{1}{c|}{82.26\%} & 82.26\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{37.60\%} & \multicolumn{1}{c|}{16.12\%} & \multicolumn{1}{c|}{16.12\%} & \multicolumn{1}{c|}{15.93\%} & \multicolumn{1}{c|}{15.93\%} & \multicolumn{1}{c|}{\textbf{13.12\%}} & \multicolumn{1}{c|}{\textbf{13.10\%}} & \textbf{13.10\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{\textbf{13.88\%}} & \multicolumn{1}{c|}{13.88\%} & \multicolumn{1}{c|}{13.88\%} & 13.88\% \\ \hline
\multirow{3}{*}{Random workload 12} & CPLEX & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{88.99\%} & \multicolumn{1}{c|}{85.96\%} & \multicolumn{1}{c|}{85.96\%} & \multicolumn{1}{c|}{85.89\%} & \multicolumn{1}{c|}{85.05\%} & \multicolumn{1}{c|}{84.00\%} & \multicolumn{1}{c|}{83.79\%} & \multicolumn{1}{c|}{82.80\%} & 82.80\% \\ \cline{2-13} 
 & GUROBI & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{37.11\%} & \multicolumn{1}{c|}{20.44\%} & \multicolumn{1}{c|}{20.32\%} & \multicolumn{1}{c|}{20.26\%} & \multicolumn{1}{c|}{20.26\%} & \multicolumn{1}{c|}{\textbf{10.23\%}} & \multicolumn{1}{c|}{\textbf{10.23\%}} & \multicolumn{1}{c|}{\textbf{10.23\%}} & \textbf{10.23\%} \\ \cline{2-13} 
 & Ours & \multicolumn{1}{c|}{100.00\%} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{\textbf{13.94\%}} & \multicolumn{1}{c|}{13.94\%} & \multicolumn{1}{c|}{13.94\%} & \multicolumn{1}{c|}{13.94\%} & 13.94\% \\ \hline
\end{tabular}%
}
\end{table*}
